An Inversion Tool for Conditional Term Rewriting Systems -- A Case Study of Ackermann Inversion

We report on an inversion tool for a class of oriented conditional constructor term rewriting systems. Four well-behaved rule inverters ranging from trivial to full, partial and semi-inverters are included. Conditional term rewriting systems are theoretically well founded and can model functional and non-functional rewrite relations. We illustrate the inversion by experiments with full and partial inversions of the Ackermann function. The case study demonstrates, among others, that polyvariant inversion and input-output set propagation can reduce the search space of the generated inverse systems.

==> eptcsdata.tex <==
\providecommand{\firstpage}{33}
\providecommand{\publicationstatus}{Alexei Lisitsa and Andrei Nemytykh (Eds.): 9th International Workshop\\ on Verification and Program Transformation (VPT 2021)\\
EPTCS 341, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.341.3}{10.4204/EPTCS.341.3}}
\pdfoutput=1

